AAMDM: Accelerated Auto-regressive Motion Diffusion Model

Interactive motion synthesis is essential in creating immersive experiences in entertainment applications, such as video games and virtual reality. However, generating animations that are both high-quality and contextually responsive remains a challenge. Traditional techniques in the game industry can produce high-fidelity animations but suffer from high computational costs and poor scalability. Trained neural network models alleviate the memory and speed issues, yet fall short on generating diverse motions. Diffusion models offer diverse motion synthesis with low memory usage, but require expensive reverse diffusion processes. This paper introduces the Accelerated Auto-regressive Motion Diffusion Model (AAMDM), a novel motion synthesis framework designed to achieve quality, diversity, and efficiency all together. AAMDM integrates Denoising Diffusion GANs as a fast Generation Module, and an Auto-regressive Diffusion Model as a Polishing Module. Furthermore, AAMDM operates in a lower-dimensional embedded space rather than the full-dimensional pose space, which reduces the training complexity as well as further improves the performance. We show that AAMDM outperforms existing methods in motion quality, diversity, and runtime efficiency, through comprehensive quantitative analyses and visual comparisons. We also demonstrate the effectiveness of each algorithmic component through ablation studies.

==> algos/DM3_sampling.tex <==
\begin{algorithm}[t]
  	\caption{DM3 Motion Generation pseudocode}
  	\label{alg:DM3_sampling}
  	\begin{algorithmic}[1]{

          \Require  Decompressor Network $D$ , Generator Network $G^{GA}$, Denoise Network $G^{DN}$, Total Diffusion Steps $T^{DM3}$ and Diffusion Steps in Denoise Module $T^{DN}$, Forward Diffusion $FD$
          \item[]

        \State Given: embedded vector $\bfx\bfz_{n-1}$ at motion step n-1
        \Repeat
        \State Check user input $\bar{\bfx}_n \leftarrow$ User input
        \State Initialize: diffusion step $t\leftarrow T^{DM3}$
        \State Initialize: generated embedded vector $\bfx\bfz^{t}_{n} \sim N(0, I)$.
         \item[]
        \State {{\textsc{// Rollout Generation Module }}}
        \Repeat
        \State Sample $r^t \sim N(0, I)$
        \If {$\bar{\bfx}_n$ is not \textit{None}}
            \State Set $\Phi(r^t) = 0$
        \EndIf
        \State Reverse Diffusion $\hat{\bfx\bfz}^{0}_{n} \leftarrow G^{GA}(\bfx\bfz^{t}_{n}, \bfx\bfz_{n-1}, r^t,t)$
        \If {$\bar{\bfx}_n$ is not \textit{None}}
        \State Update $\hat{\bfx\bfz}^{0}_{n}$ using Equation \ref{equ:guided_diffusion}
        \EndIf
        \State Forward Diffusion  $\bfx\bfz^{t-1}_{n} \leftarrow FD(\hat{\bfx\bfz}^{0}_{n})$
        \State $t \leftarrow t-1$
        \Until{$t = T^{DN}$}

        \item[]
        \State {{\textsc{// Rollout Denoise Module }}}
        

        \Repeat
        \State Reverse Diffusion $\hat{\bfx\bfz}^{0}_{n} \leftarrow G^{DN}(\bfx\bfz^{t}_{n}, \bfx\bfz_{n-1}, r^t,t)$
        \If {$\bar{\bfx}_n$ is not \textit{None}}
        \State Update $\hat{\bfx\bfz}^{0}_{n}$ using Equation \ref{equ:guided_diffusion}
        \EndIf
        \State Forward Diffusion  $\bfx\bfz^{t-1}_{n} \leftarrow FD(\hat{\bfx\bfz}^{0}_{n})$
        \State $t \leftarrow t-1$
        \Until{$t = 0$}
        \item[]

        \State {{\textsc{// Decompress to Full Pose Vector }}}
        \State $\bfx\bfz_{n} \leftarrow \hat{\bfx\bfz}^{0}_{n}$ 
        \State$\bfy_n \leftarrow D(\bfx\bfz_{n})$
        \State$n \leftarrow n+1$

        \Until{desired}

        }
  	\end{algorithmic}
\end{algorithm}

==> paper_text/method_old.tex <==


\section{Overview}
In this work, we introduce \dmmm (\textbf{D}iffusion \textbf{M}odels for \textbf{M}otion \textbf{M}atching), a scalable and efficient approach for interactive synthesizing character motions. An overview of the method is depicted in Figure \ref{fig:DM3_Overview}. \sehoon{I think we can improve the overview. Figure 1 looks a bit complicated. Can you first illustrate the rough architecture of MM, LMM, Diffusion, and our method? Then we can provide a more detailed overview, which is the current Figure 1.} Our framework generate motion with the following procedure. \sehoon{Again, this is too abrupt. You can explain the key invention of our method over the existing algorithms.} At each time instance, the previous embedded vector $\bfx\bfz_{ n-1 } $ and the user input $ \bar{\bfx}_n $ are used to produce the current embedded vector $ \bfx\bfz_{n} $ through a learned Stepping model. Then, the pose vector $ \bfy_n $ is constructed by a learned Decompressor network $ D $ from $ \bfx\bfz_{n}$. The predicted embedded vector $ \bfx\bfz_{n}$ is then used in an auto-regressive manner for future poses generation. Overall, the motion generation procedure is similar to Learned Motion Matching(\textbf{LMM}) ~\cite{LearnedMotionMatching} with the main variation being how we model the Stepping and how we address the user's query $ \bar{\bfx} $.

\tianyu{Not sure if we should list the shortage of LMM here, to justify why we propose a methods }


Specifically, in \textbf{LMM}, the Stepping model is a single neural network a.k.a Stepper, and \textbf{LMM} uses a separate network a.k.a  Projector to map the user's query $ \bar{\bfx} $ to embedded vector $\bfx\bfz_{n}$. \sehoon{The previous sentence can be cleaned up.} However, \dmmm uses a single Stepping model, which we name it as Diff-Stepper to include the function of both Stepper and Projector. The Diff-Stepper uses a diffusion model sampling procedure to generate new embedded vector $\bfx\bfz_{n}$. \sehoon{Why is this important?} Given embedded vector in previous motion step $\bfx\bfz_{ n-1 }$, Diff-Stepper samples a random noise vector $\bfx\bfz^T_{n}$, then iterate from T to 1. At each diffusion step t, Diff-Stepper predicts the clean sample $\hat{\bfx\bfz}^0_{n}$ \sehoon{what does it mean by a clean sample? Is it a technical term?} and diffuses it back to $\hat{\bfx\bfz}^{t-1}_{n}$. The Diff-Stepper is consist \sehoon{check grammar} of two modules: a Denoise Module and a Generation Model. The Denoise Network $G^{DN}$ in the Denoise Module takes  The Generation Module uses Denoising Diffusion-GANs~\cite{DiffGAN} formulation where a Generator Network takes $\bfx\bfz_{n-1}$, $\bfx\bfz_{n}$ and diffusion step $t$ as input, whereas the Generator Network $G^{GA}$ in the Generation Module take an additional vector $r^t$ to model each denoising step using a multimodal conditional GAN for fast synthesis ~\cite{DiffGAN}. We use the query from the user $ \bar{\bfx} $ to guide the generation process such that the generated pose $y_n$ can meet the requirement. \sehoon{overview is a bit confusing. We need a better structure.}


\section{Diffusion Models for Motion Matching}
There are three target properties that our proposed method should fulfill:
\begin{itemize}
    \item The system should be able to replicate the various motions within the motion data.
    \item The generation time shouldn't be too long and the generation process shouldn't use massive memory.
    \item The motion generated should meet the user's commands.
\end{itemize}
To achieve high-quality motion generation, \dmmm employs a low-dimensional embedded vector in place of a high-dimensional pose vector, simplifying the pose transition learning process. Additionally, it utilizes an Autoregressive Diffusion Model to capture the many-to-many nature of pose transitions in the dataset. To facilitate efficient motion synthesis, \dmmm leverages the Denoising Diffusion-GAN technique to accelerate the diffusion model sampling procedure. Finally, to ensure controllability, \dmmm is trained with a regularization term and uses a gradient-based objective function to guide the generation result to meet the user's query. Further details on these techniques will be provided in the following subsections.


\subsection{Constructing Low-dimensional Embedded Space}
The first step in DM3 is constructing a low-dimensional embedded space $\mathbf{XZ}$ from the full pose space $\mathbf{Y}$. The main motivation of this step is to make learning step inference easier. We will demonstrate this claim in Section \ref{sec: baseline_comparison}.

To construct the embedded space, we use a similar autoencoder-based method as in ~\cite{LearnedMotionMatching}. Specifically, we create a Compressor network $C$ and a Decompressor network $D$. The Compressor network projects a pose $\mathbf{y}_n$ to a low-dimensional vector $\bfz_n$. The Decompressor network then aims to reconstruct $\mathbf{y_n}$ from the feature vector $\mathbf{x}_n$ and $\mathbf{z}_n$. The embedded space is defined as the concatenation of the feature vector and projected vector $\mathbf{xz}_n$. The Compressor and Decompressor network are trained together to minimize visually perceived error and regularization losses on $Z$. Please refer to ~\cite{LearnedMotionMatching} for a detailed design of the loss function. Once the two networks are trained, we compute $z_n$ for each frame n and store the embedded vector collection $\mathbf{XZ} = [\mathbf{xz}_0, \mathbf{xz}_1, \cdots, \mathbf{xz}_N]$ using the Compressor network.  Once the embedded vector space is created, we thus convert the motion generation problem from learning a full-state Stepping model $S(\mathbf{y}_{n-1}) \rightarrow \mathbf{y}_{n} $ to embedded state Stepping model $S(\mathbf{xz}_{n-1}) \rightarrow \mathbf{xz}_{n} $. And the generate pose can be constructed with the trained Decompressor network $D(\mathbf{xz}_{n}) \rightarrow \mathbf{y}_{n}$.


\subsection{Autoregressive Diffusion Model for Sequential Generation}
Now that our goal is to train Stepping model for autoregressive embedded vector prediction. In LMM ~\cite{LearnedMotionMatching}, this Stepping model is represented by a neural network trained with a MSE-based objective function. This method assumes a one-to-one mapping between $ \mathbf{xz}_{n-1} $ and $ \mathbf{xz}_{n} $. However, this assumption can be violated when the dataset contains plenty of motions, where one motion poses can have multiple candidate following poses. The many-to-many poses mapping problem trigger us to leverage diffusion model to tackle this problem.


Our diffusion model follows the structure of DDPM ~\cite{ho2020denoising} introduced in Section \ref{sec: bg_diffusion}. Specifically, during the forward diffusion process for each diffusion step, a small noise vector is added on top of the future embedded vector $\mathbf{xz}_{n}$ after T steps:
\begin{equation}
    q(\mathbf{xz}^{t}_{n} | \mathbf{xz}^{t-1}_{n}) = N(\sqrt{\alpha^t} \mathbf{xz}^{t-1}_{n}, (1-\alpha^t)I),
\end{equation}
where $\alpha^t \in (0,1)$ are constant parameters. If T is large enough $\mathbf{xz}^T_{n}$  is equivalent to an isotropic Gaussian noise $N(0, I)$. 

The reverse phase is modeled as gradually removes the noise given the previous embedded vector $\mathbf{xz}_{n-1}$ to generate the prediction of $\mathbf{xz}_{n}$. Instead of predicting the noise added as used by ~\cite{ho2020denoising, shi2023controllable}, in our setting we follow ~\cite{ramesh2022hierarchical, tevet2022human} and predict the vector directly with the objective function:
\begin{equation}
\label{equ:diff}
   L = \mathbb{E}_{t\sim [1,T]} [||\mathbf{xz}_{n} - \mathbf{\hat{xz}}^0_{n}||] = [||\mathbf{xz}_{n} - G^{DN}_\theta(\mathbf{xz}^t_{n},\mathbf{xz}_{n-1}, t)|| ]
\end{equation}
The predicted $\mathbf{\hat{xz}}^0_{n}$ is then used as condition for generating next embedded vector $\mathbf{xz}_{n+1}$. For training the Autoregressive Diffusion Model instead of using objective function \ref{equ:diff}. We use the similar objective function in \textbf{LMM} to ensure high quality generation over long horizon:
\begin{equation}
\label{equ:denoise_module_loss}
   L^{DN} = w_{Xval}L_{Xval} + w_{Zval}L_{Zval} +w_{Xvel}L_{Xvel} + w_{Zvel}L_{Zvel}
\end{equation}
where for feature vector $\bfx$:
\begin{align}
L_{Xval} =  |\bfx_{n:n+h} - \hat{\bfx}^0_{n:n+h}| \\
L_{Xvel} =  |(\bfx_{n:n+h} - \bfx_{n-1:n+h-1}) -(\hat{\bfx}^0_{n:n+h}-\hat{\bfx}^0_{n-1:n+h-1})|
\end{align}
and we apply the same manner to $\bfz$.

Although our diffusion model generation process looks similar to A-MDM ~\cite{shi2023controllable}, there are two main difference between our Autoregressive Diffusion Model and A-MDM. Firstly, we use diffusion model for generating embedded vector while A-MDM generates full pose vector. A lower conditionality has the benefit of easier to learn, less memory usage and faster prediction speed. Secondly, A-MDM predicts the noise added on the vector while our model directly predicts the vector. 

However, although diffusion model own the good property such as high quality samples and excellent mode coverage, it suffers from long sampling time due to the back and forth diffusion and denosing procedure, therefore prohibit it usage for real-time motion generation.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/DD_GANs.pdf}
    \caption{Overview of DD-GANs.}
    \label{fig:DD-GANs_overview}
    \vspace{-0.5cm}
\end{figure}



\subsection{Fast Generation via Denoising Diffusion-GANs}
The reason that Diffusion Model takes many steps for denoising is that the denoising distribution is assumed to be Gaussian distribution. This Gaussian assumption holds only in the infiniesimal limit of tiny denoising steps ~\cite{DiffGAN}, thus leads to the need of a large number of reverse process. If we want the reverse process uses fewer steps, we need a non-Gaussian multimodal distribution for modeling the denoise distribution.

To tackle this challenge, we leverage Denoising Diffusion-GANs(DD-GANs) proposed by Xiao et al ~\cite{DiffGAN}. This approach formulate the reverse diffusion process using an expressive multimodal distribution. This is achieved by parameterized the reverse diffusion process conditional GANs, where the reverse diffusion generator $G^{GA}$ takes an additional variable $r^t$ as input:
\begin{align} 
   \hat{\mathbf{xz}}^0_{n} = G^{GA}_{\theta'}(\mathbf{xz}^t_{n},\mathbf{xz}_{n-1},\mathbf{r}^t ,t)
\end{align}
We use $G^{GA}(\sim)$ as an abbreviation of $G^{GA}_{\theta'}(\mathbf{xz}^t_{n},\mathbf{xz}_{n-1},\mathbf{r}^t ,t)$.
The training objective for the generator $G^{GA}$ is to minimize the divergence between two distributions:
\begin{align}
    min_{G^{GA}} [Div(p_{\theta’}(\mathbf{xz}^{t-1}_n|\mathbf{xz}^{t}_n, \mathbf{xz}_{n-1})\ 
    ||\  q(\mathbf{xz}^{t-1}_n|\mathbf{xz}^{t}_n, \mathbf{xz}_{n-1}))]
\end{align}
This objective can then be converted to training a diffusion-step-dependent discriminator network $D^{SC}_\phi(\mathbf{xz}^{t-1}_n, \mathbf{xz}^{t}_n, \mathbf{xz}_{n-1}, t)$ to distinguish if $\mathbf{xz}^{t-1}_n$ is diffused from the original data or generated fake data $\hat{\mathbf{xz}}^0_{n}$, and the generator is trained to cheat the discriminator. We use $D^{SC}(\sim)$ as an abbreviation of $D^{SC}_\phi(\mathbf{xz}^{t-1}_n, \mathbf{xz}^{t}_n, \mathbf{xz}_{n-1}, t)$. The training objective for the discriminator $D^{SC}$ and the generator $G^{GA}$ can be summarized as
\begin{multline}
\label{equ:dis_loss}
    L_{D^{SC}} \ = \; -\mathbb{E}_{q(\mathbf{xz}^{t-1}_n|\mathbf{xz}^{t}_n, \mathbf{xz}_{n-1})}[log(D^{SC}(\sim)] \\
     -\mathbb{E}_{p_{\theta’}(\mathbf{xz}^{t-1}_n|\mathbf{xz}^{t}_n, \mathbf{xz}_{n-1})}[log(1-D^{SC}(\sim))]
\end{multline}
\begin{align}
    L_{G^{GA}} = -\mathbb{E}_{p_{\theta’}(\mathbf{xz}^{t-1}_n|\mathbf{xz}^{t}_n, \mathbf{xz}_{n-1})}[log(D^{SC}(\sim))]
\end{align}
Figure \ref{fig:DD-GANs_overview} is an illustration of the DD-GANs framework, please refer to \cite{DiffGAN} for more details.

DD-GANs provides us with high sampling(generation) speed while keeps the excellent mode coverage and output quality of in a single motion steps. However, we observe that using DD-GANs for our autoregressive generation setting will lead to unstable training procedure that deteriorate the resulted motion output.

\input{algos/DM3_training}

\subsection{Combining Diffusion Model and Denoising Diffusion GANs}
To enjoy the both high sampling speed introduced by DD-GANs while take advantage of the motion quality of the Diffusion model in the autogressive setting, we proposed a framework, \textbf{Diff-Stepper} that combines these two methods.Diff-Stepper is composed by a Generation Module and a Denoise Module. The Generation Module is based on DD-GANs and is used for generate embedded vector in few reverse diffusion steps. The Denoise module is used for improve the quality of embedded vector that generate by the Generation Module for autoregreesive motion generation. The Generation Module is concatenated with the Denoise Module. The reverse diffusion sampling contains $T^{GA}$ steps for fast generation then the output is sent to the Denoise Module and go through $T^{DN}$ steps for polishing result. Here, $T^{DN} << T^{Diff}$  The total sampling steps of Diff-Stepper is the sum of generation sampling steps and denoise sampling steps $T^{DM3} = T^{GA}+T^{DN}$ These design leads Diff-stepper capable of generating high-quality output with short sampling time. 

Training Diff-stepper contains two major components. First, training the Denoise Module using the same procedure as the Autoregressive Diffusion Model procedure. Then, train the Generation Module using the $\bfx\bfz_{n-1}$ generated by rollout out trained Denoise Module. For specifc training procedure please refer to Algorithm \ref{alg:DM3_training}.



\input{algos/DM3_sampling}

\subsection{Controll Motion Synthesis via Guided Diffusion}
To generate the motions that follow user's commands, for single pose transition, DM3 guides the motion generation process through a guided diffusion method proposed by Rempe ~\cite{rempe2023trace}. Given the user's query $\bar{\bfx}_n$, at each diffusion steps with noise vector $\bfx\bfz^t_{n}$, we perturb the generated vector $\hat{\bfx\bfz}^0_{n}$:
\begin{align}
\label{equ:guided_diffusion}
    \hat{\bfx\bfz}^{0,*}_{n} = \hat{\bfx\bfz}^0_{n} - \epsilon \alpha^t \nabla_{\bfx\bfz^t_{n}} J(\hat{\bfx}^0_n, \bar{\bfx}_n).
\end{align}
Here, $J$ is an objective function measuring distance between the generated feature vector and user's query. $\epsilon$ is a step parameter, $\alpha^t$ is the noise parameter in diffusion model.

Beside guided diffusion, we also introduce a regularization term for training $G^{GA}$ in Generation Module, the total objection for $G^{GA}$ becomes:
\begin{multline}
\label{equ:gen_net_loss}
    L_{G^{GA}} = -\mathbb{E}_{p_{\theta’}(\mathbf{xz}^{t-1}_n|\mathbf{xz}^{t}_n, \mathbf{xz}_{n-1})}[log(D^{SC}(\sim))] +\\ w_{reg}(|\hat{\bfx}^0_n - \bfx^t_n|- |\Phi(r^t)| )^2.
\end{multline}
Here, $\Phi(r^t)$ is the subspace of the addition variable $r^t$ in DD-GANs and $w_{reg}$ is a weight parameter. The interpretation of the regularization term is that we want some $\Phi(r^t)$ corresponds to less variation in $\bfx$. Therefore, we can manually set $\Phi(r^t)$ to zero vector when we are required to meeting user's command. A summary of control procedure are summarized in Alorithm: \ref{alg:DM3_sampling}.






% In LMM, the ‘matching’ of input feature vector  $\mathbf{\bar{x}}_n$ is achieve via an additional network aka Projector trained to emulate the nearest neighbor search behavior. The additional network introduce extra training procedure while increase the memory usage. Here, we used a Conditional Inpainting to control the embedded vector generation. The Conditional Inpainting can be simply implement by replace generated embedded vector at reverse diffusion step t, $\mathbf{\hat{xz}}^{t}_n$ with $\mathbf{\bar{x}\hat{z}}^{t}_n$ in the Generation Module. We found that this simple design is practical for matching the input feature vector $\mathbf{\bar{x}}_n$ to proper $\mathbf{\hat{xz}}^{0}_n$.

==> paper_text/user_study.tex <==
\section{User Study}

Follow commands

If you like
